RM-Bench: Benchmarking Reward Models of Language Models with Subtlety and Style

Reward models are critical in techniques like Reinforcement Learning from Human Feedback (RLHF) and Inference Scaling Laws, where they guide language model alignment and select optimal responses. Despite their importance, existing reward model benchmarks often evaluate models by asking them to distinguish between responses generated by models of varying power. However, this approach fails to assess reward models on subtle but critical content changes and variations in style, resulting in a low correlation with policy model performance. To this end, we introduce RM-Bench, a novel benchmark designed to evaluate reward models based on their sensitivity to subtle content differences and resistance to style biases. Extensive experiments demonstrate that RM-Bench strongly correlates with policy model performance, making it a reliable reference for selecting reward models to align language models effectively. We evaluate nearly 40 reward models on RM-Bench. Our results reveal that even state-of-the-art models achieve an average performance of only 46.6%, which falls short of random-level accuracy (50%) when faced with style bias interference. These findings highlight the significant room for improvement in current reward models. Related code and data are available at https://github.com/THU-KEG/RM-Bench.

==> section/0-abs-bak.tex <==


% Reinforcement learning (RL) plays a crucial role in aligning large language models (LMs) with human preferences, as evidenced by systems like ChatGPT. 

% Despite the growing significance of reward models in this process, their evaluation remains under-explored. 

% Existing benchmarks lack comprehensive testing of style bias and often fail to correlate with policy model performance. 

% To address this, we propose \ourbench, a novel benchmark designed to assess reward models in real-world scenarios, incorporating style bias evaluation and correlating closely with policy model outcomes. 

% \ourbench tasks models with selecting the better response from two generated outputs for a given prompt, covering a wide range of domains including Chat, Safety, Code and Math.
% % Using diverse datasets and generating varied response styles, we construct a robust evaluation set filtered by human annotators. 

% Extensive experiments demonstrate that \ourbench strongly correlates with policy model performance during both training and inference. 

% We evaluate over 40 reward models, including classical sequence-classification models and newly proposed multi-objective models, alongside chat models trained with Direct Policy Optimization (DPO). 

% Our results show that even state-of-the-art reward models struggle on \ourbench, underscoring the need for improved benchmarks in this domain.
% 

\begin{abstract}
Reward models are critical in techniques like Reinforcement Learning from Human Feedback (RLHF) and Inference Scaling Laws, where they guide language model alignment and select optimal responses. 
However, existing methods often rely on comparisons between responses from models of varying power, failing to assessing reward model with subtle but critical changes and style variations.
In this work, we introduce \ourbench, a novel benchmark designed to evaluate reward models on their sensitivity to subtle content differences and resistance to style biases. 
% Our benchmark uses responses generated by the same model, GPT-4o, with rejected responses incorporating subtle errors and a range of styles. 
Extensive experiments demonstrate that \ourbench strongly correlates with policy model performance, making it a reliable reference when selecting reward models for alignment of language models.
We evaluate nearly 40 reward models on \ourbench.
Experiments show that even state-of-the-art reward models only achieve a random-level (50\%) performance of 46.6\% under the interference of style bias, indicating significant room for improvement.

% only 46.6\% under the interference of style bias, indicating significant room for improvement.
% with struggle to exceed random-level performance under the style interference, with 46.6\%
% revealing significant room for improvement.
% We find that \ourbench highlights the significant improvement needed for reward models,
% with even state-of-the-art reward models struggling to exceed random-level performance under the style interference.
%  and reveals significant room for improvement.
% We find that current reward models, even large-scale ones like Nemotron-340B-Reward, struggle to tell 
% Additionally, models trained with Direct Policy Optimization (DPO) outperform sequence-classification reward models, suggesting DPO’s potential for advancing reward model performance.
\end{abstract}

==> section/1-intro_bak.tex <==

% The remarkable achievements of Large Language Models (LLMs) such as ~\citep{} are largely predicated on Reinforcement Learning from Human Feedback (RLHF)~\citep{}. The core of RLHF lies in the objective of aligning language models with human-centered preferences~\citep{}, which is captured by reward modeling~\citep{}. During the reward modeling process, a reward model is initially optimized on preference datasets~\cite{} and will then provide a preference label on candidate texts based on predefined criteria during inference. Consequently, reward models assume a pivotal role in assessing preference quality, thereby directly influencing the performance of the aligned models (policy models) they optimize.

% Despite the significant position in aligning policy models, benchmarking the performance of reward models remains underexplored especially compared with the recent efforts on assessing policy models~\citep{} and pretrained models~\citep{}. This would impede the community from an in-depth understanding of the reward model performance and thereby increase the potential cost in preference alignment. Therefore, it is necessary to steer our attention and promote the emphasis on assessing reward models.

% To conduct a faithful and systematical evaluation, we curate the benchmark based on three principal properties: 1) \textbf{Awareness of Subtle Changes:} A faithful reward model should provide preference based on the text factuality~\citep{} , meaning that it can discriminate chosen and rejected responses even if the change is subtle (e.g. in Table 1 the chosen and rejected responses only differentiate in few words while expressing totally opposite meanings). 2) \textbf{Robustness against Style Bias:} Previous studies~\citep{} have indicated the susceptibility of language models to style bias. For instance, simply adding bold symbols of markdown to the response would completely mislead the reward model’s preference. Therefore, a robust reward model should resist these spurious correlations and judge the response primarily on its semantic meaning. 3) {Correlation with Policy Models:} Given that policy models are guided by rewards from reward models, the quality of the reward models should authentically reflect the capabilities of the policy models. This implies that the performance of reward models should exhibit a positive correlation with the downstream evaluation of policy models.

% In line with our studies, recent efforts~\citep{lambert2024rewardbench,starling2023,llm-blender-2023} have made progress by constructing benchmarks from existing preference datasets. Typically, these benchmarks involve providing a prompt and two responses, asking the reward model to assign a higher reward to the better response. However, compromising in construction cost, they often use responses from a powerful LM as the better response and generate a worse response from a weaker LM, which may not reflect the application scenario of the reward model. This could lead to reward models hacking with the style of powerful LMs, rather than focusing on the content quality and results a low correlation with the aligned language model performance~\citep{ivison2024unpacking}, highlighting the need for a more refined benchmark that can better evaluate reward models.





% To this end, we propose RM-Bench, a high-quality reward model benchmark towards faithfully and systematically evaluating reward models under the application-aligned scenario. RM-Bench explicitly models the impact of style biases and also manifests a strong correlation with policy model performance. In particular, for property 1): Given a large output space, randomly curating chosen and rejected responses is inefficient. Therefore, it is necessary to select critical evaluation examples to genuinely reflect the performance of reward models in open-ended problems. We achieve it by intentionally designing \textit{hard} response pairs by introducing only subtle changes for evaluation. This would facilitate the general evaluation of reward models which can extrapolate the performance to those unseen responses that are easy to classify; for property 2): Considering the potential impact from biases, we adopt two representative spurious features~\cite{arena}, including the response length and markdown format as they are likely to dominant the models’ decision as evident by previous studies~\cite{}. Our evaluation provides the deceptive preference selection caused by style biases as a proof of concept and can be applied to more biases in future explorations; for property 3): In addition to solely evaluating the reward models on RM-Bench, we further consider the correlation between performance of reward and policy models and conduct extensive experiments on RM-Bench. This makes our benchmark more practical in real-world scenarios. 

% Finally, we evaluate over 40 mainstream reward models on \ourbench, including sequence-classification reward models, multi-objective reward models, and chat models trained with Direct Policy Optimization (DPO)~\citep{cui2023ultrafeedback, adler2024nemotron, rafailov2023direct}.
% Our results highlight several key findings:
% 1) \textit{There is substantial progress needed in enhancing reward model performance.} As indicated by our experiments, even the giant reward models, such as Nemo-340B-Reward~\citep{adler2024nemotron}, struggle on \ourbench, indicating there is still room for improvement in reward models.
% 2) \textit{Style biases deserve more attention in faithfully evaluating reward models.} When predicting rewards, the reward models are easily interfered with by the style of the responses, yaws from the substance of responses.
% 3) \textit{DPO models demonstrate more potentials in reward modeling.} The DPO models compared to its sequence-classification counterparts, demonstrate a better performance on \ourbench, suggesting that DPO models could be a potential candidate for reward models.
% 4) \textit{Reward models should avoid being evaluated in isolation.} Since the ultimate goal is to align policy models with reward models, reward models with higher performance should have positive impacts on the downstream assessment of policy models.



% \newpage
\section{Introduction}
\label{sec:intro}
The remarkable achievements of Large Language Models (LLMs) such as ChatGPT, Claude, and OpenAI o1~\citep{chatgpt,bai2022training,openai_o1_preview} is highly relied on Reinforcement Learning from Human Feedback~\citep[RLHF,][]{ouyang2022training,bai2022constitutional}
or Inference Scaling Law~\citep{snell2024scaling,wu2024empirical,lightman2023let}.
Reward models play a pivotal role in both two techniques above. 
In RLHF, reward models serve as a proxy of human value to provide feedback on generated text, which is used to align language models, namely the policy model, during training~\citep{ouyang2022training,dong2024rlhf}.
% provide feedback on generated text, which can be used to align language models wi
% during training~\citep{ouyang2022training,dong2024rlhf}.
And in Inference Scaling Law, reward models help to select the best response from a set of candidate responses based on its predicted rewards~\citep{wu2024empirical,snell2024scaling}.
% Reward models play a pivotal role in optimizing large language models (LMs) by providing feedback on generated text, which can be used to align language models during training through Reinforcement Learning with Human Feedback \citep[RLHF,][]{ouyang2022training,llama3modelcard,chatgpt} and improve language model performance at inference by providing rewards to the generated text~\citep{openai_o1_preview, wu2024empirical,snell2024scaling}.
% Systems like ChatGPT and Claude~\citep{chatgpt,bai2022training} have highlighted the effectiveness of reward models in aligning LMs with human preferences, making them more responsive and practical in real-world applications.

Despite their significance, benchmarks for evaluating reward models remain under-explored compared to the rapid advancements in language model evaluation~\citep{hendrycks2020measuring, srivastava2023beyond, chiang2024chatbot, hendrycksmath2021}.
To conduct a faithful and systematical evaluation, an ideal benchmark for reward models should adhere to three key principles:
1) \textbf{Assessing Reward Models' Sensitivity to Subtle Changes:}
% Evaluating reward models' sensitivity to subtle changes in responses.
A faithful reward model should sensitively distinguish this change and assign higher reward to the correct response.
For example, in Table~\ref{tab:example-data}, Response 1 and Response 2 only differ in one word but express totally different meanings requiring the reward model to focus on the content quality.
2) \textbf{Assessing Reward Models' Robustness against Style Biases:}
% 2) \textbf{Assessing Reward Models under Style Interference:}
% Evaluating reward models' robustness against style biases.
A robust reward model should resist these spurious correlations between style and content and always reject the response with factual errors regardless of its style.
For example, in Table~\ref{tab:example-data}, Response 3 is factually incorrect, but more lengthy than Response 1, misleading the reward model to assign a higher reward to Response 3.
3) \textbf{Correlating with Policy Models:}
A good reward model benchmark should have a high correlation with the performance of the post-RLHF model, namely, the policy model.
Thus, it can serve as a reliable proxy for finding the best reward model for RLHF training.


% 1) \textbf{Application-aligned:} The benchmark should reflect real-world use cases, such as in Proximal Policy Optimization (PPO)~\citep{schulman2017proximal} and Best-of-N sampling~\citep{wu2024empirical}, where all candidate responses are generated by the same LM.
% 2) \textbf{Sytle Unbiased evaluation:} The evaluation should provide unbiased measurements of reward model abitilies preventing the reward model from hacking the intrinsic biases in the benchmark.
% 2) \textbf{Style Controlled evaluation:} The benchmark should provide a style controlled evaluation to avoid reward model hacking the bench from style shortcut between chosen responses and different responses.
% 3) \textbf{Policy model correlation:} The benchmark should be highly correlated with performance on the aligned language model, namely, the policy model.
% ~\footnote{In context of Reinforcement Learning of language models, the policy model refers to the language model being aligned, in this paper, we use the term aligned language model and policy model interchangeably.}.

Recent efforts~\citep{lambert2024rewardbench,starling2023,llm-blender-2023} have made progress by constructing benchmarks from existing preference datasets.
Typically, these benchmarks involve providing a prompt and two responses,
asking the reward model to assign a higher reward to the better response. 
However, compromising in construction costs, they often use responses from a powerful LM as the better response, and generate the worse response from a weaker LM.
This design choice fails to assess the reward model's ability to distinguish subtle changes in responses since the responses are generated by different LMs.
This could also lead to reward models hacking with the style of powerful LMs, failing to assess the reward model's ability to resist style biases.
These two issues could result in a low correlation with the aligned language model's performance~\citep{ivison2024unpacking}, highlighting the need for a more refined benchmark that can better evaluate reward models.
% which may not reflect the application scenario of the reward model.
% This could leads to reward models hacking with the style of powerful LMs, rather than focusing on the content quality and results a low correlation with the aligned language model performance~\citep{ivison2024unpacking}, highlighting the need for a more refined benchmark that can better evaluate reward models.

To this end, we propose a new benchmark, \ourbench, towards evaluating reward models' ability to distinguish subtle changes and resist style biases.
In particular,
1) To evaluate reward models' sensitivity to subtle changes, we construct both the chosen and rejected responses with the same LM, gpt-4o~\citep{openai_gpt4o}.
The rejected responses contains subtle errors which are introduced by jailbreaking or multi-sampling.
2) To evaluate reward models' robustness against style biases, we use dedicated style-controlled prompts to construct responses with different styles including concise, detailed, and markdown-formatted.
3) Finally, we conduct extensive experiments to show that \ourbench has a high correlation with the policy model's performance in both the training and inference process.

% the application-aligned scenario, avoiding the style shortcuts and providing a high correlation with the policy model's performance.
% In particular, 1) To align with the application scenario of reward models, we construct the both two responses with the same LM, gpt-4o~\citep{openai_o1_preview}.
% 2) To avoid the style shortcuts, we use dedicated style-controlled prompts to construct responses with different styles including concise, detailed, well-formatted.
% 3) Finally, we conduct extensive experiments to show that \ourbench has a high correlation with the aligned language model's performance in both the training and inference process.

\input{table/0-example-data.tex}



Finally, we evaluate nearly 40 various reward models on \ourbench, including sequence-classification reward models, multi-objective reward models, and chat models trained with Direct Policy Optimization (DPO)~\citep{cui2023ultrafeedback, adler2024nemotron, rafailov2023direct}.
Our results highlight several key findings:
% TODO: NEED LISTING?
1) \textit{There is substantial progress needed in enhancing reward model performance.} As indicated by our experiments, even the giant reward models, such as Nemotron-340B-Reward~\citep{adler2024nemotron}, struggle on \ourbench, indicating there is still room for improvement in reward models.
2) \textit{Style biases deserve more attention in faithfully evaluating reward models.} When predicting rewards, the reward models are easily interfered with by the style of the responses, yaws from the substance of responses.
3) \textit{DPO models demonstrate more potential in reward modeling.} The DPO models compared to its sequence-classification counterparts, demonstrate a better performance on \ourbench, suggesting its potential as a candidate for reward models.
% DPO models could be a potential candidate for reward models.
% 4) \textit{Reward models should avoid being evaluated in isolation.} Since the ultimate goal is to align policy models with reward models, reward models with higher performance should have positive impacts on the downstream assessment of policy models.


% Finally, we evaluate nearly 40 reward models on \ourbench, including sequence-classification reward models, multi-objective reward models, and chat models trained with Direct Policy Optimization (DPO)~\citep{cui2023ultrafeedback, adler2024nemotron, rafailov2023direct}.
% Our results reveal that:
% 1) Even the giant reward models, such as Nemo-340B-Reward~\citep{adler2024nemotron}, struggle on \ourbench, indicating there is still room for improvement in reward models.
% 2) When predicting rewards, the reward models are easily interfered by the style of the responses, yaws from the substance of responses.
% 3) The DPO models compared to its sequence-classification counterparts, demonstrate a better performance on \ourbench, suggesting that DPO models could be a potential candidate for reward models.


% To summarize, our contributions are as follows:
% \begin{itemize}[leftmargin=*,topsep=0pt,itemsep=1pt,parsep=0pt]    
%     \item We identity the three key principles for an ideal benchmark for reward models: application-aligned, unbiased evaluation, and policy model correlation.
%     \item Follow these principles, we propose a new benchmark, \ourbench, where each prompts are combined with two set of responses with different styles all generated by gpt-4o.
%     \item Extensive experiments shows that existing reward models are easily interfered by the style of the responses, even the giant reward models, Nemo-340B-Reward, struggle on \ourbench, indicating there is still room for improvement in reward models.
% \end{itemize}









